DPGen: Automated Program Synthesis for Differential Privacy

Differential privacy has become a de facto standard for releasing data in a privacy-preserving way. Creating a differentially private algorithm is a process that often starts with a noise-free (non-private) algorithm. The designer then decides where to add noise, and how much of it to add. This can be a non-trivial process -- if not done carefully, the algorithm might either violate differential privacy or have low utility. In this paper, we present DPGen, a program synthesizer that takes in non-private code (without any noise) and automatically synthesizes its differentially private version (with carefully calibrated noise). Under the hood, DPGen uses novel algorithms to automatically generate a sketch program with candidate locations for noise, and then optimize privacy proof and noise scales simultaneously on the sketch program. Moreover, DPGen can synthesize sophisticated mechanisms that adaptively process queries until a specified privacy budget is exhausted. When evaluated on standard benchmarks, DPGen is able to generate differentially private mechanisms that optimize simple utility functions within 120 seconds. It is also powerful enough to synthesize adaptive privacy mechanisms.

==> alg_svt.tex <==
\begin{figure}[!ht]
\setstretch{0.9}
\raggedright
\small
\noindent\rule{\linewidth}{0.8pt}
\funsigfour{SVT}
{\code{T,N,size}\annotation{:\tyreal_0}, $q$\annotation{:\tylist~\tyreal_*}}
{(\code{out}\annotation{:\tylist~\bool}), \bound{\priv}}
{\alldiffer}
\algrule
\begin{lstlisting}[frame=none,escapechar=@,basicstyle=\appendixalgsize\ttfamily]
$\eta_1$ := $\lapm{(2/\priv)}$
$\tT$ := $T + \eta_1$;
count := 0; i := 0;
while (count < N $\land$ i < size)
  $\eta_2$ := $\lapm{(4N/\priv)}$
  if ($\text{q[i]}+\eta_2\geq \tT$) then
    out := true::out;
    count := count + 1;
  else
    out := false::out;
  i := i + 1;
\end{lstlisting}
\noindent\rule{\linewidth}{0.8pt}
\funsigthree{Transformed SVT}
{\code{T,N,size,q}\instrument{, \code{\distance{q}}, $\noise$, $\hole$}}
{(\code{out})}
\algrule
\begin{lstlisting}[frame=none,escapechar=@,firstnumber=12,basicstyle=\appendixalgsize\ttfamily]
@\instrument{$\vpriv{\priv}$ := 0; idx = 0;}@
@\instrument{$\eta_1$ := $\noise$[idx]; idx := idx + 1;}@
@\instrument{$\vpriv{\epsilon}$ := $\vpriv{\epsilon}$ + $|\alignment_1| \times \priv / 2$; \distance{$\eta_1$} := $\alignment_1$;}@
$\tT$ := $T$ + $\eta_1$;
@\instrument{\distance{$\tT$} := \distance{$\eta_1$};}@
count := 0; i := 0;
while (count < N $\land$ i < size)
  @\instrument{$\eta_2$ := $\noise$[idx]; idx := idx + 1;}@
  @\instrument{$\vpriv{\priv}$ := $\vpriv{\priv}$ + $|\alignment_2| \times \priv / 4N$; \distance{$\eta_2$} := $\alignment_2$;}@
  if (q[i] + $\eta_2$ $\geq$ $\tT$) then
    @\instrument{\assert{q[i] + $\eta_2$ + \distance{q}[i] + \distance{$\eta_2$} $\geq$ $\tT$ + \distance{$\tT$}};}@
    out := true::out;
    count := count + 1;
  else
    @\instrument{\assert{$\lnot$(q[i] + $\eta_2$ + \distance{q}[i] + \distance{$\eta_2$} $\ge$ $\tT$ + \distance{$\tT$})};}@
    out := false::out;
  i := i + 1;
@\instrument{\assert{$\vpriv{\priv} \le \priv$};}@
\end{lstlisting}
\noindent\rule{\linewidth}{0.8pt}
\caption{Standard Sparse Vector Technique and its transformed code, where underlined parts are added by \tool. The transformed
code contains two alignment templates for $\eta_1$ and $\eta_2$:
$\alignment_1 = \hole[0]$ and $\alignment_2 = (\code{q[i] +
$\eta_2$[i] $\ge$ $\tT$})\mathbin{?}(\hole[1] + \hole[2] \times
\distance{$\tT$} + \hole[3] \times
\distance{\code{q}}\code{[i]})\mathbin{:}(\hole[4] + \hole[5] \times \tT +
\hole[6] \times \distance{\code{q}}\code{[i]})$.\label{alg:svt}}
\end{figure}

==> reviews.tex <==
Comments

- [x] First, given that the paper builds significantly on top of existing approaches like [44], I suggest adding some more details explaining the new ideas (sections 3.2 and 4.2).

- [x] Moreover, the presentation of the transformation rules from [44] (section 4.1) is very difficult to follow due to a lack of details. This is problematic because understanding how the transformation works is critical to understand both DPGen and the examples given in the paper.

- [x] Finally, it'd be nice to have a few more details about (1) how the while-priv construct works in the context of [44] (is it a simple extension or it requires significant changes?), and 

- [x] I found section 4.1 very difficult to follow and understand. The authors give only extremely high-level details which are not sufficient to understand how the program transformation works. In particular, the entire "reasoning about privacy" paragraph seems to consist of background from [44] (given that the only new rule seems to be the T-While-Priv explained in section 4.3). The lack of details, however, makes it rather unhelpful for a reader. For instance, these are a few (important) aspects that I couldn't figure out without reading [44]:

- [x] How do alignment templates look like? How can they be generated?

- [x] The rule T-Laplace is pretty confusing and even after skimming through

- [x] (2) how users can select good utility functions (the one provided for adaptive SVT is rather complex, so I'm wondering how realistic would it be to expect users to come up with them in the first place).
    
- [x] [44] I have a few doubts. In particular, the assertion $c_a$ seems to be
    expressed over pairs of executions (I guess to ensure alignment) where
    $\eta_1, \eta_2$ seem to both refer to $\eta$'s value in the two runs.
    However, (1) the assertion seems to be added to the original program rather
    than to the transformed one in T-Laplace, and (2) it's unclear how such
    assertions could be expressed in the transformed program since the
    transformed program (e.g., in figure 7) does not seem to contain primed
    variables for the two executions (like in self-composed programs).

- [x] Rules T-Asgn and T-Return refer to a $\mathcal{C}$ in the assert
        statement, but $\mathcal{C}$ is unbound.

- [x] The paper states that the rules are the same as those in [44].
        However, the transformation rules for expressions produce judgments
        $\Gamma \vdash e : \mathcal{B}_{\mathbb{n}} | \mathcal{C}$ in [44] and
        judgemnts of the form $\Gamma \vdash e : \mathcal{B}_{\mathbb{n}}$ in
        Figure 18.

- [x] Does the new T-While-Priv rule require changes to [44] proof/key insights
    or is it a rather simple extension?

- [x] Section 4.2 is one of the key contributions of the paper since Section 4.1 is
heavily based on CheckDP. However, the authors only give high-level details
about the synthesis loop and mechanism generation. I suggest adding some more
details (e.g., How are problems encoded for PSO?)

- [x] The idea of using taint-tracking to identify potential locations for injecting
noise is very nice. However, I suggest adding a a step-by-step discussion of the
example (e.g., what are the tainted variables? what are the offending
variables?) to clarify how the approach works.

- [ ] Section 3.2.3 states that noise is injected before the declaration and use
    of offending variables. Given this, I do not understand why the algorithm
    would inject the noise on lines 2-3 since variables i and count should be
    untainted (count is conditionally updated based on private inputs, but the
    taint-tracking does not track implicit flows) and size and N are
    non-private. What am I missing?\yuxin{I think the reviewer confused tainted variables with offending variables? But I think the paper is pretty clear on this subject...}

- [x] Unless I missed something tainted variables are a subset of offending
    variables, right? If yes, stating this explicitly might help a bit the
    reader.

- [x] I like that DPGen uses the utility function to balance the amount of inserted
noise. However, as pointed out by the authors the default utility function might
not always be the best choice. Are there general principles that users should
follow to select a "good" utility function? More generally, is there a way of
characterizing good utility functions?

- [x] Experiments: In the comparison with Kolahal (last column in Table 1), are the
algorithms whose result is N/A supported by Kolahal (but numbers are not
reported in [38]) or are they not supported?

- [x] "miss of randomness" --> "lack of randomness"

- [x] Improve presentation of section 4.1. The authors should give enough
information for the reader to be able to (at least) understand how the examples
in the paper are generated.

- [x] It is hard to understand the shape of alignment templates and how they are generated. The paper uses the function GenerateTemplate, but without given any intuition on how it works. Is this exactly the same GenerateTemplate function as CheckDP? Did you need it to adapt it? If so, how? (see my comment about the delta w.r.t. previous work) What is the type of alignment templates? Please,
  clarify these aspects.

- [x] This work takes as a baseline many of the techniques developed by CheckDP. It was not totally clear to me how much authors borrow from CheckDP "infrastructure." I can see that taint analysis, and while-priv rule being novel here. However, I cannot get an appreciation about how much the CEGIS algorithm (also used by CheckDP) was needed to be changed (if and how).

- [x] The utility optimization routine completes the synthesis picture but I couldn't appreciate how this part works. Is it a black-box optimization that you just plugged in into the pipeline in Fig. 8? How would authors say that from the Table 1, the synthesis algorithm obtained a good utility for the considered examples?

- [x] Determining the sensitivity of the queries is crucial to produce an appropriate noise scale; for simplicity, DPGen assumes the user will pass this information as an input. It is unclear how DPGen can generate a correct noise scale when the given sensitivities are inconsistent (e.g., wrongly indicating that an average has sensitivity 1).

- [x] In section 4.2 is mentioned that soundness checks are meant to be done using CheckDP in a future integration. Still, the authors claimed that none of the synthetized programs were unsound; it would be worth mentioning whether such a statement comes from either passing all results through CheckDP or any other kind of soundness check.

- [x] How do you check the soundness on while-priv loops since CheckDP does not support them?

- [x] What is the intuition behind starting with a search space in the alignment of [-10,10] and the holes scale [0,10]?

- [x] Fig. 1: q hat is not introduced until Page 5.

- [x] Page 4: you talk about lambda holes to be synthesized in phase 2, but in phase
  2 you talk about theta holes. Please, clarify that there are two different kinds of holes upfront.

- [x] Fig 4: How do you represent empty lists?

- [x] Fig 6: where are eta1 and eta2 coming from? I guess that you refer to the two
  (relational) executions


- [x] Why do you focus only on the Laplace mechanism? Is combining multiple mechanisms difficult with your approach?

- [x] The computation of the privacy cost of a candidate program relies on the composition theorem. It is known that this theorem provides privacy bounds which are not necessarily tight. Could it be that because of this, DPGen will return a sub-optimal program? That is, DPGen will return a program that meets the privacy cost requirements, but its utility is lower than another private program P, because the composition theorem will (wrongfully) state that P’s privacy cost is larger than the required cost? It would be helpful to discuss this point and maybe present a (non-private) program for which DPGen returns a sub-optimal solution. 

- [x] I found Section 2 confusing because it combined background and overview. I’d suggest moving subsections 2.5 and 2.6 to a separate section (called Overview).

- [x] Section 4 header should be "synthesis and optimization".

- [x] Page 7, right, first paragraph: Lines 3, 8, 10 (not 3, 9, 11).

- [x] The paper assumes that sensitivity is provided by the user. It's not really
clear to me how big of a deal that is. Will this make it hard to apply DPGen to
new algorithms? That is, will we have to use DPGen in tandem with a technique
for proving sensitivity bounds? Or is this something we can easily determine, looking
at the problem. Can we use a conservative approximation? It would be nice to
have a bit more discussion on this.

- [x] In Section 2.1 sensitivity comes a bit out of nowhere; the notion of query f
is also introduced quite abruptly.

- [x] I found 2.2 a bit difficult to follow in detail. For instance, it's not clear
to me, what are the requirements on alignment functions in general, and what they
look like, in practice. Also, the bound on privacy cost could use a bit more
explanation. I found this part hard to follow. Of course, all of this is background and covered in other papers, but it would be good to be as self-contained as possible.

- [x] In Figure 4, I find the use of star a bit confusing. It's used to denote
private variables before, but here it just serves to mark the new set of
commands in the target language?

- [ ] In Section 3.2, when computing offending variables, in principle, there could
be a longer chain of definitions leading from private inputs to the usage site.
I imagine, one could add any of these variables to the offending set, broadening
the space of possible privacy mechanisms. But I guess this might blow up solving
time? \yuxin{I think we \_are\_ collecting all offending variables along the chain of definitions, which the paper is also quite clear...}

- [x] Seeing the general definition of alignment function, I assume the templates
only cover a subset of possible alignment functions? It's of course fine as long
as they include proofs for interesting programs.

- [x] Speaking of alignment functions, it's not clear to me how function
GenerateTemplate works. I think this part of the method overlaps with CheckDP,
so maybe there are more details there, but it would be nice to add more
explanation in the paper. For example, how are we choosing which branch
conditions to include in the template? This is not entirely clear to me.

- [x] Also in Section 4.1: it seems, the assertions should include an assertion
stating that the difference in output is zero. This is not needed for this
example, but, it seems, would be required in general.

- [x] I appreciate the discussion on soundness.

- [x] It would be interesting to apply DPGen to a new algorithm to see, if a privacy mechanism can be found. What would be the hard parts in doing this? Coming up with a sensitivity estimate?
Maybe alignment functions would be needed that cannot be expressed through the templates?
Or maybe, in some cases, Laplacian noise is not enough? A discussion on this would be very valuable to the reader.

- [x] Intro: From utility perspective -> From a utility perspective.

- [x] 3.2, first paragraph: the miss of randomness -> the lack of randomness.

- [x] How hard is it for the user to provide sensitivity as input?

==> sec_synthesis.tex <==




